Quantum computer specification for nuclear structure calculations

Recent studies to solve nuclear structure problems using quantum computers rely on a quantum algorithm known as Variational Quantum Eigensolver (VQE). In this study, we calculate the correlation energy in Helium-6 using VQE, with a \textit{full-term} unitary-paired-coupled-cluster-doubles (UpCCD) ansatz on a quantum computer simulator and implement a set of custom termination criteria to shorten the optimization time. Using this setup, we test out noisy quantum computer simulators of various coherence times and quantum errors to find the required specification for such calculations. We also look into the contribution of errors from the quantum computers and optimization process. We find that the minimal specification of 5~ms coherence times and $10^{-4}$ quantum errors is required to reliably reproduce state-vector results within 8\% discrepancy. Our study indicates the possibility of performing VQE calculations using a full-term UpCCD ansatz on a slightly noisy quantum computer, without implementing quantum error correction.

==> notused/notadding.tex <==
\section{Introduction}
%Quantum computing offers a new computing paradigm, utilizing the quantum properties, presenting computing resources not accessible by classical computing, here classical computer refers to digital computation that represent information by basic unit of information bit described as either one of two static states; qubit in quantum computer however represents the superposition of the two states.
\red{Need a new introduction before talking about algo.. bla bla bla.} 
An example of a promising application of quantum computers is [quantum algorithm]. 
In the noisy intermediate-scale quantum (NISQ) era, where quantum processing unit (QPU) is susceptible to high error rate and limited qubit coherence times, algorithms requiring deep quantum circuits such as quantum phase estimation (QPE) is challenging to implement effectively.
\blue{Alternative class of algorithm known as Variational Quantum Eigensolvers (VQE)~\cite{Peruzzo2014}, requires less quantum operations, holds promise to solve eigenvalue problem before arrival of fault tolerant quantum computer.}


%However, exploratory work is necessary to prepare ourselves for fault-tolerant quantum computers. # too generic

%Our work focuses on the application of variational quantum eigensolver (VQE)~\cite{Peruzzo2014} in solving for nuclear pairing correlation in $^6$He nucleus.

% There are several models of quantum computing e.g.~quantum annealing model and measurement based quantum computation (MBQC)~\cite{Nimbe2021, Briegel2009}.
% This paper concerns only of the unitary circuit model, also known as quantum circuit model.
% Of which the essential part of the computation involves building of unitaries to represent the quantum state and observable, whose expectation value is evaluated by repeated measurement of the quantum circuit, also known as shot.

VQE is a hybrid quantum-classical algorithm that solves for the expectation value of an observable $\hat{A}$ of a system via classically minimization of a Ritz-Rayleigh functional, also known as cost function, in the form of quantum circuits. Take the example of an operator to be minimised to be a Hamiltonian $\hat{H}$, the ground state solution $E_0$ associated with the Hamiltonian is bounded by the cost function given by
\begin{equation}
    E_{0} \leq
    \frac{\left\langle \psi\left( \left\{ \theta_i\right\} \right) \right\vert 
    \hat{H}\left\vert 
    \psi\left( \left\{ \theta_i \right\} \right) \right\rangle }
    {\left\langle \psi\left( \left\{\theta_i\right\} \right)
    |\psi\left( \left\{\theta_i \right\} \right) \right\rangle }
    \label{eq:VQE cost function}
\end{equation}
where the $\left\vert \psi \left( \left\{ \theta_i \right\}\right)\right\rangle$ are unitary ansatz state as a function of a set of parameters $\left\{ \theta_i\right\}$, and represented on quantum computer as parameterised quantum circuits. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{plt0031/vqe illustration.png}
    \caption{}
    \label{fig:enter-label}
\end{figure}
The cost function in equation~\eqref{eq:VQE cost function} is minimised by a classical optimizer, where in each step of minimization or iteration, the expectation value of the cost function will be evaluated using a quantum computer, and using the information of the expectation value, the parameters of for the cost function is updated for the next iteration.
For each evaluation, a quantum computer would prepare and measure many shots of this expectation value circuits to obtain a statistic for a good enough expectation value.
VQE algorithm would repeat the minimization steps until it satisfy termination criteria, e.g. reaching maximum number of iteration defined or achieving convergence threshold. 
Variations of VQE exist, being different in the structure of ansatz and strategies for optimization, which are extensively reviewed in Ref.~\cite{Tilly2022}.

In nuclear physics, shell model correlated ground state constructed using VQE had been studied on nuclei $^6$He, $^8$Be, $^{20}$O and $^{22}$O by considering an inert core and valence nucleons interacting via Cohen-Kurath interaction~\cite{Stetcu2022}. % cite this in (https://www.nature.com/articles/s41598-023-39263-7)
Similar study has been done also with $^6$Li nucleus~\cite{Kiss2022}, on the effect of ordering of fermionic excitation operators within the unitary coupled cluster. 
Both the studies consider inert core to limit the number of qubits required, with the same spirit, our study focuses on small nuclei needing only QPU with small number of qubits.

This work \red{is somewhat similar to Refs. ~\cite{Stetcu2022, Kiss2022}, sci.fic.}, where we start with a meanfield solution--referring to meanfield microscopic description of nucleonic system--which is very similar to other correlated quantum problems, thus sharing some of the approaches to build correlated states.
Resource intensive full configuration interaction (FCI), allow for an exact to numerical precision solution of Schr\"{o}dinger's equation, which can be used as a benchmark for quantum many-body correlation~\cite{Lietz2017}.
Less intensive alternatives like the coupled cluster theory allows for larger basis of single-particle states not possible in FCI.
In nuclear physics, other frameworks offer to build wavefunction ansatz correlated to the Hartree-Fock (HF) ground state, such as the Hartee-Fock-Bogoliubov (HFB) approximation~\cite{Decharg1980,Dobaczewski1984}, or its Bogoliubov-Valatin limit yielding wavefunctions the BCS theory~\cite{Kennedy1964}, highly truncated diagonalization approach~\cite{Pillet2002, Laftchiev2010}, Random Phase approximation~\cite{Stetcu2002}, etc.

Here, we calculate the pairing correlation interaction in $^6$He nucleus within unitary coupled cluster doubles using VQE algorithm. 
% This paper concerns about the residual interaction calculation with initial solution generated from microscopic meanfield calculation. 
\red{Pairing correlation interaction is considered as one of many types of residual interaction and is also the main interest within the meanfield community.}

\red{highlight investigation of FakeJohors.}

This paper is organised as follows. First, we describe Hartre-Fock meanfield approach, frameworks to account for residual interaction and coupled cluster theory in Sec.~\ref{sec:theory}. 
Quantum computing implementation of coupled cluster theory is detailed in Sec.~\ref{sec:qc implementation}, that includes the mapping of the Hamiltonian and UpCCD ansatz, and the construction of the cost function. 
In Sec.~\ref{sec:Results and discussions}, results from statevector simulation and noisy simulator are included. 
We presented several simulated noisy quantum computer with customised noise model in Sec.~\ref{sec:fakeJohors}
Results from other IBM noisy simulators are presented in the Appendix. 

\section{Theoretical Framework\label{sec:theory}}
As one of the fields that deals with quantum many body problems, nuclear physics suffers from curse of dimensionality among other quantum mechanical problems. 
One of the approaches is using Hartree-Fock meanfield approach, reducing the many body problem into a problem of single particle in an average potential.
Phenomenological interaction such as Skyrme interaction that deals with neutron and proton degree of freedom reproduces experimental data and is often used as an alternative. 
This study focuses on using the phenomenological effective Skryme interaction with SLy4 parameterization, solved using HF approach.

The converged meanfield solution is as good as the HF approach can get.
Higher order interactions are considered as residual interaction, in the field of nuclear microscopic theory, meanfield community typically consider pairing interaction for the residual interaction. 
This section elaborates on general implementation of HF approach considering Skryme interaction and how the pairing correlation energy can be accounted for by using the BCS framework and finally the modification to coupled cluster theory to build paired-unitary coupled cluster doubles (p\-UCCD) anstaz that mimics the pairing behavior.

\subsection{The Hamiltonian and HF Reference Solution \label{sec:HF,residual,CCT}}
\subsubsection{Skryme Two-body Effective Interaction}
The two-body interaction is taken to be of Skyrme type~\cite{Skyrme1958} with its full form described in Appendix~\ref{skyrme two-body interaction}.
The SLY4 parameterizations used in this study  \textcolor{red}{parameterizations~\cite{Beiner1975}, for its good spectroscopic characteristic that performs well in predicting nucleus on the line of stability.} The non-zero parameters in the unit of $\text{MeV}\cdot \text{fm}^{3}$ are given by 
\begin{center}
\begin{tabular}{|l|r|}
 \hline
 \hline
Parameter & SLy4    \\
\hline
$t_0$ (MeV fm$^3$)  & -2488.910  \\
$t_1$ (MeV fm$^5$)  & 486.820    \\
$t_2$ (MeV fm$^5$)  & -546.390   \\
$t_3$ (MeV fm$^{3+3\sigma}$)  & 13777.000 \\
$x_0$               & 0.834 \\
$x_1$               & -0.344    \\
$x_2$               & -1.000    \\
$x_3$               &  1.354    \\
$\sigma$            & $\frac{1}{6}$   \\
$W_0$ (MeV fm$^5$)  &   123.000 \\
% Parameter & SIII      \\
% t0        & -1128.75  \\
% t1        & 395.00    \\
% t2        & -95.00    \\
% t3        & 14000.00    \\
% x0        & 0.45     \\
% W         & 120.00     \\
 \hline
 \hline
\end{tabular}
\end{center}

\subsubsection{HF Meanfield Approximation}
HF approximation assumes a $A$-body system to be a system of independent particles, with the each particle moving in an average one-body potential contributed by the rest of the $\left(A-1\right)$ particles. Essentially, reducing the problem of $A$-body system into a particle in a potential well problem. 

A general Hamiltonian that includes only up to two-body interaction for a $A$-nucleon nucleus is given by
\begin{align} % Second quantised form
    H&=\sum_{i}t_i + \sum\limits_{i<j} V_{ij},
    \label{eq:General Hamiltonian short}
\end{align}
or in second quantised form
\begin{multline}
    H=\sum_{\alpha \beta }\left\langle \alpha \right\vert t\left\vert \beta
    \right\rangle a_{\alpha }^{\dagger }a_{\beta }\\
    +\frac{1}{2}%
    \sum\limits_{\alpha \beta \gamma \delta }\left\langle \alpha \beta
    \right\vert V\left\vert \gamma \delta \right\rangle a_{\alpha
    }^{\dagger }a_{\beta }^{\dagger }a_{\delta }a_{\gamma },
    \label{eq:General Hamiltonian}
\end{multline}
where $T$ is kinetic energy and $V$ is the two-body interaction operators; and the state $\left\vert \alpha \right\rangle$, $\left\vert \beta \right\rangle$, $\left\vert \gamma \right\rangle$, and $\left\vert \delta \right\rangle$ form an arbitrary complete set. 

equation~\eqref{eq:General Hamiltonian} can be rewritten as
\begin{equation}
    H = \sum_{i}^{A}h_{\text{SP}} + \left[\sum_{i<j}V_{ij} - \sum_{i}U_{i} \right]
    = H_{\text{MF}} + V_{\text{res}},
    \label{eq: MF + RES}
\end{equation}
where the meanfield Hamiltonian $H_{\text{MF}}$ sums over the single-particle Hamiltonian $h_{\text{SP}}$. 
The single-particle Hamiltonian that generates the single-particle states $\left\vert l\right\rangle$, $\left\vert m\right\rangle$, $\left\vert n\right\rangle$, \dots, and $\left\vert a\right\rangle$, $\left\vert b\right\rangle$, $\left\vert c\right\rangle$, \dots, is given in second-quantised form as \cite{Preston_Bhaduri_1993}
\begin{equation}
\label{eq:HF hamiltonian}
    h_{\text{SP}}=\sum_{ki}^{A}\left[ \left\langle k\right\vert t\left\vert
    i\right\rangle +\left\langle k\right\vert U\left\vert i\right\rangle \right]
    a_{k}^{\dagger }a_{i},
\end{equation}
where the occupied single particle states are denoted with $\left\vert l\right\rangle$, $\left\vert m\right\rangle$, $\left\vert n\right\rangle$, \dots, while the unoccupied states are denoted by $\left\vert a\right\rangle$, $\left\vert b\right\rangle$, $\left\vert c\right\rangle$, \dots; and the matrix element of one-body meanfield potential $U$  between orbitals $r$ and $s$, 
\begin{equation}
\label{eq:HF average(mean) field}
    \left\langle r\right\vert U\left\vert s\right\rangle
    =\sum\limits_{m=1}^{A}\left( \left\langle rm\right\vert V\left\vert
    sm\right\rangle -\left\langle rm\right\vert V\left\vert ms\right\rangle
    \right),
\end{equation}
are contributed by the $A$  occupied orbitals $\left\vert m\right\rangle$, generated from the two-body force $V$ be it an actual or phenomenological interaction.

The HF solution demands self-consistency, that a set of trial single-particle orbitals is first chosen and those which are occupied are selected to calculate the one-body potential in equation~\eqref{eq:HF average(mean) field}. Then the equation~\eqref{eq:HF hamiltonian} is solved to generate a new set of single-particle orbitals, the procedures are repeated until the solution converge.

The ground state solution to the $A$-body system in HF approximation is assumed to be a single Slater Determinant $\left\vert \Phi\right\rangle$, constructed from the converged single-particle orbitals, with the lowest energy state filled up first. The ground-state energy with the HF ground state $\left\vert \Phi_{0}\right\rangle$, is given by
\begin{equation}
    E_{\text{HF}} = \sum^{A}_{l=1} \left[ e_l -\frac{1}{2}\left\langle l \right\vert U \left\vert l \right\rangle \right],
    \label{eq:Hartree-Fock Energy}
\end{equation}
where $U$ is defined in equation~\eqref{eq:HF average(mean) field}, and the factor of $\frac{1}{2}$ comes from the double counting of the potential.

For a HF approximation to be a good one, the residual interaction $V_{\text{res}}$ in equation~\eqref{eq: MF + RES} should be small compared to the $E_{\text{HF}}$. Higher order interactions\textemdash{two-body pairing correlations} as residual interaction will be described in the next section.

% \textcolor{red}{\textbf{Rearrangement energy}}
% In the case where the two-body interaction $V$ is density dependent, a correction term $C$ is included in the terms of  equation~\eqref{eq: MF + RES} where the meanfield Hamiltonian Hamiltonian $H_{MF}$ is rewritten as
% \begin{align}
%     H_{\text{MF}} &=\sum_{i}^{A} \left( t_{i} + U_{i}\right) + C,\\
%     V_{\text{res}} &= \sum_{i<j}V_{ij} - \sum_{i}U  - C,
% \end{align}
% where $t$ and $U$ are as defined on the previous part, the correction term is given by 
% \begin{equation}
%     C = E_\text{R} - \left\langle \Phi_{0}\right\vert \hat{V} \left\vert \Phi_{0}\right\rangle,
% \end{equation}
% the rearrangement energy $E_R$ as described in Eqs. (38) and (39) from Ref.~\cite{Vautherin1972} is
% \begin{equation}
%     E_\text{R} = -\frac{1}{12}\sum_{ijk}\left\langle ijk\right\vert\bar{v}_{123}\left\vert ijk\right\rangle.
% \end{equation}

\subsection{Residual pairing interaction\label{sec:Residual interaction}}
The residual interaction can take several forms.
In the meanfield community, pairing correlation interaction is typically considered, other correlation may includes vibrational correlation~\cite{Nadja2010}.N

Given a pairing interaction $V_{12}\left(\mathbf{r}\right)$, the matrix elements are defined by the integral over the volume of the nucleus $\Omega$ % \cite{Preston_Bhaduri_1993} %Eq8.93
\begin{widetext}
    \begin{equation}
        \left\langle \mathbf{k}_{i}\left( 1\right) ,-\mathbf{k}_{i}\left( 2\right)
        \right\vert V_{12}\left\vert \mathbf{k}_{i}^{\prime}\left( 1\right) ,-%
        \mathbf{k}_{i}^{\prime}\left( 2\right) \right\rangle  
        = \frac{1}{\Omega }\int \exp \left( i\mathbf{q} \cdot \mathbf{r}\right) V_{12}\left( \mathbf{r}\right)d^3r,
        \label{eq:pairing matrix element}
    \end{equation}
\end{widetext}
where $\mathbf{q} = \mathbf{k}_{i}^{\prime} - \mathbf{k}_{i}$ is the centre of mass momentum and $\mathbf{r} = \mathbf{r}_1 - \mathbf{r}_2$ is the distance between the 2 particles.

The extreme case of density-dependent delta interaction which is also a state-dependent interaction takes the form of~\cite{Preston_Bhaduri_1993}
\begin{equation}
    V_{12}\left(\mathbf{r}\right) = -G\Omega\delta \left( \mathbf{r}\right),
    \label{eq:dddi pairing}
\end{equation}
reduces equation~\eqref{eq:pairing matrix element} to 
\begin{equation}
    \left\langle \mathbf{k}_{i}\left( 1\right) ,-\mathbf{k}_{i}\left( 2\right)
    \right\vert V_{12}\left\vert \mathbf{k}_{i}^{\prime}\left( 1\right) ,-%
    \mathbf{k}_{i}^{\prime}\left( 2\right) \right\rangle   = - G
\end{equation}
where $G$ is the pairing matrix.

In this study, we consider the simplest form of pairing interaction matrix\textemdash{the seniority force}, which has constant antisymmetrised matrix elements of
\begin{equation}
    G = \frac{V_{0}}{11+N_{\tau}}=\text{const},
    \label{eq:seniority pairing}
\end{equation}
$N_{\tau}$ represent the number of nucleon, where $\tau$ represents the 2 possible isospin state\textemdash{either proton state or neutron states}, and $V_{0}$ represents pairing strength fitted from experimental data.

From equation~\eqref{eq: MF + RES}, the more general form of Hamiltonian with residual pairing correlation interaction may be rewritten as
\begin{equation}
    H =\sum_{v}e_{v}\hat{a}_{v}^{\dagger }\hat{a}_{v}+\frac{1}{4}\sum\limits_{ij\Tilde{kl}}V_{ijkl}\hat{a}_{i}^{\dagger}\hat{a}_{j}^{\dagger }\hat{a}_{l}\hat{a}_{k},
    \label{eq:pairing_hamiltonian}
\end{equation}
where $e_{v}$'s are the single-particle energies of nucleons in the average potential $U$, $V_{ij\Tilde{kl}}$ is antisymmetrised pairing matrix element, and $\hat{a}^\dagger$ and $\hat{a}$ are the fermionic creation and annihilation operators; the factor $\frac{1}{4}$ is made up of the $\frac{1}{2}$ from the double counting where the sum over $i,j,k,l$ is not restricted, and another $\frac{1}{2}$ for the antisymmetrised matrix element $V_{\mu\bar{\nu}}$.
\subsubsection{HF+BCS framework}
Several approaches are available to build many-body basis to describe the correlated states. 
HFB and HF+BCS theory, commonly used for their simplicity to implement, are plagued by their properties of not conserving the particle number, a trade off for the simplicity.
Another framework akin to truncated shell model calculation is the HTDA~\cite{Nadja2010}, which unlike BCS framework, preserves the particle number with the higher computation cost.

In BCS framework, the ansatz solution are constructed from quasiparticle vacuum state $\left\vert0\right\rangle$
\begin{equation}
    \left\vert \text{BCS}\right\rangle =\prod_{\mu >0}\left( u_{\mu }+v_{\mu }a_{\mu
    }^{\dagger }a_{\bar{\mu}}^{\dagger }\right) \left\vert 0\right\rangle 
\end{equation}
where $\left\vert 0\right\rangle$ is vacuum state, and the occupation probability of pair states $\left(\mu ,\bar\mu\right)$ is described by the value of $v_{\mu}^{2}$ and probability of the states being empty is $u_{\mu}^{2}$, with assumptions that there are no correlation between pairs and $\mu$ represents quantum number $n,l,j,m$.

To find the BCS ground state, one minimize variationally the expectation value of $\left\langle\text{BCS}\right\vert H^{\prime
}\left\vert \text{BCS}\right\rangle $ with respect $v_{\mu }$ to obtain finding the parameters $u_{\mu }$ and $v_{\mu }$. The Hamiltonian $H^{\prime}$ in the expectation value is modified from equation~\eqref{eq:pairing_hamiltonian},
\begin{equation}
    H^{\prime }=\sum_{v}\left( e_{v}-\lambda \right) \hat{a}_{v}^{\dagger }\hat{a%
    }_{v}-G \sum_{\mu ,\nu>0}\hat{a}_{\mu }^{\dagger }\hat{a}_{\bar{\mu}}^{\dagger }%
    \hat{a}_{\bar{\nu}}\hat{a}_{\nu},
\end{equation}
where here in the HF+BCS framework, $e_{v}$'s are the single-particle energies of nucleons in the average potential $U$ obtained from HF approximation %preston Eq. 8.97
, $\lambda $ is a lagrange multiplier taken to be the chemical potential of the system% check page 323 of preston's
, and $\mu>0$ refers to states with consideration of only $m>0$.
%the $G$ is \textcolor{red}{Check preston's eq 8.92}

The pairing gap energy of the minimised $\left\vert \text{BCS}\right\rangle$ state is given by
\begin{equation} % preston's page 320, eq 8.108
% SHould i use the word/symbol of gap energy or just E_pair
    \Delta_{gap}=-G\sum_{\mu>0}u_{\mu}v_{\mu}.
\end{equation}

\subsubsection{Coupled Cluster Theory}
Coupled cluster ansatz is written with an exponential generator acting on a reference state $\left\vert\Phi_{0}\right\rangle$,
\begin{equation}
\label{eq:CCT ansatz}
\left\vert \psi \right\rangle =e^{\hat{T}}\left\vert \Phi _{0}\right\rangle ,
\end{equation}%
where for inclusion of only singles and doubles coupled clusters operators give us
\begin{equation}
\label{eq:SD cluster operators}
\hat{T}=\hat{T}_{1}+\hat{T}_{2}
\end{equation}%
with 
\begin{align}
    \hat{T}_{1}&=\sum_{ia}t_{i}^{a}\hat{a}_{a}^{\dagger}\hat{a}_{i},
    \label{eq:1h1p excitation}\\
    \hat{T}_{2}&=\sum_{ijab}t_{ij}^{ab}\hat{a}_{a}^{\dagger }\hat{a}
    _{b}^{\dagger }\hat{a}_{j}\hat{a}_{i}\label{eq:double excitation}.
\end{align}where \eqref{eq:1h1p excitation} and \eqref{eq:double excitation} represent 1-hole-1-particle and 2-hole-2-particle excitation respectively. The indices $a,b$ represent particle state and $i,j$ represent hole states, the coefficients $t_{i}^{a}$ and $t_{ij}^{ab}$ are to be found out for the correlation energy.

Within the quantum circuit computation model, state and observable are built as unitary quantum circuits, thus modification on \eqref{eq:CCT ansatz} has to be done such that
\begin{equation}
    \left\vert \psi \right\rangle =e^{\hat{T}-\hat{T}^\dagger}\left\vert \Phi _{0}\right\rangle, \label{eq:UCC ansatz}
\end{equation}
which is the unitary coupled cluster (UCC) ansatz, which will be converted into parameterised quantum circuit, as a wavefunction ansatz correlated to the HF ground state. Variations of UCC ansatz exist such that they are different by inclusion of different excitation cluster operators, e.g. singles excitation operators includes only one-hole-one-particle excitation, other more advanced structure is studied in Ref.~\cite{Lee2018}.

Pairing effect in nuclear physics has been studied using coupled cluster theory~\cite{Henderson2014, Stein2014}, in the form of pair coupled cluster doubles (p-CCD), which is equivalent to AP1roG~\cite{Limacher2013}.
The p-CCD ansatz includes only double excitation cluster operators that do not break pairs.
Similarly, this study concerns only the double excitations to mimic the effect of pairing, where the nucleons are excited in pairs. Only terms in equation~\eqref{eq:double excitation} that excite nucleons in pair are considered. 

In this paper, the set of optimised parameters $t^{ab}_{ij}$ are to be found via variational minimization of the pairing Hamiltonian~\eqref{eq:pairing_hamiltonian} via the VQE framework.
\red{To obtain the pairing correlation energy $E_{\text{pair}}$, the expectation value of the observable $V_{\text{pair}}$ which is the second term of equation~\eqref{eq:pairing_hamiltonian} is evaluated with the optimised wavefunction ansatz $\psi_{\text{opt}}$ with the parameter $\vec{\theta}_{\text{opt}}$ such that
\begin{equation}
    E_{\text{pair}} = \left\langle\psi_{\text{opt}}\right\vert \hat{V}_{\text{pair}} \left\vert\psi_{\text{opt}}\right\rangle
\end{equation}
}

\section{QC Implementation\label{sec:qc implementation}}
In this study, we use VQE from the Qiskit library~\cite{Qiskit}, which is completed with all the basic modules, requiring only some modification, allowing us to focus on studying the pairing interaction using UCC ansatz framework. 
                                                                           
In this section, mapping of the pairing correlation interaction on a quantum computer will be described.

\subsection{Mapping onto VQE algorithm}
The quantum computing part of VQE is the evaluation of expectation value of the cost function~\eqref{eq:VQE cost function} made up of unitary quantum circuits composed of the ansatz and Hamiltonian corresponding to the quantum state and observable. The Hamiltonian~\eqref{eq:pairing_hamiltonian} and the wavefunction ansatz have to be mapped into Pauli operators\textemdash{the form that can be constructed as quantum circuit}.

Encoding the cost function onto the quantum computer in the first quantised form takes up too much resource, second quantization or the occupation number representation is more suited to be implemented on near term quantum computing devices.
Several types of mapping are available, e.g.~Parity~\cite{Seeley2012-fx} and Bravyi-Kitaev~\cite{Bravyi2002-qh} mapping methodology, Jordan-Wigner mapping is chosen for easy implementation and its intuitive representation for further analysis, e.g.~each qubit represents each orbital.

In a typical calculation, Slater determinant wavefunction is constructed to represent anti-symmetrised wavefunction, satisfying the Pauli exclusion principle.
It is too expensive to build Slater determinant states on a quantum computer. Jordan-wigner mapping takes care of this by demanding the the anti-commutation relation of the creation and annihilation operators, by
\begin{equation}
    \hat{a}_i\hat{a}_j^\dagger = - \hat{a}_j^\dagger\hat{a}_j.
\end{equation}
So that, Jordan-Wigner maps fermionic operators to Pauli operators by the following map
\begin{align}
    \hat{a}_{j}^{\dagger } &\rightarrow \frac{X_{j}-iY_{j}}{2}\otimes
    Z_{j-1}\otimes ...\otimes Z_{0}, \label{eq:creation operator map}\\
    \hat{a}_{j} &\rightarrow \frac{X_{j}+iY_{j}}{2}\otimes Z_{j-1}\otimes
    ...\otimes Z_{0}.  \label{eq:Jordan wigner annihilation operator map}
\end{align}

\subsection{Constructing Expectation Value circuit}
The fermionic Hamiltonian \eqref{eq:pairing_hamiltonian} is mapped into its qubit equivalent with the transformation (\ref{eq:creation operator map},~\ref{eq:Jordan wigner annihilation operator map}), as a sum of Pauli strings, $\hat{P}_a \in \left\{ I, X, Y, Z \right\}^{\bigotimes N}$ with $N$ the number of qubits. The qubit Hamiltonian is written as
\begin{equation}
    \hat{H}_{\text{qubit}} = \sum^{\mathcal{P}}_a \omega_a\hat{P}_a
\end{equation}
where $\omega_a$ is the weight contributed from the matrix elements of the fermionic Hamiltonian and $\mathcal{P}$ is the number of Pauli strings in the Hamiltonian and at the same time the number of circuit. 

To note, the computation becomes expensive when the $\mathcal{P}$ become prohibitively large, where for each expectation value evaluation $\mathcal{P}\times N_{s}$~circuits have to be prepared and measured, here $N_s$ is the number of shots generating the statistic for expectation value. 
The number of quantum circuit can be reduced by grouping Pauli strings into sets of Abelian group, where in each set the Pauli strings can be simultaneously diagonalised through a unitary rotation of the measurement basis. 

The ansatz UpCCD is prepared by approximating the exponential generator with only pair excitations in \eqref{eq:UCC ansatz} to first order trotterized form,
\begin{equation}
    e^{\hat{T}-\hat{T}^\dagger} =\prod\limits_{abij}e^{\theta _{ij}^{ab}\hat{
    \tau}_{ij}^{ab}},
\end{equation}
where $\theta^{ab}_{ij}$ is the parameters for pair excitation cluster operators
\begin{align}
    \hat{\tau}_{ij}^{ab} &= \hat{a}_{a}^{\dagger }\hat{a}_{b}^{\dagger }\hat{%
    a}_{j}\hat{a}_{i}-\hat{a}_{i}^{\dagger }\hat{a}_{j}^{\dagger }\hat{a}_{b}%
    \hat{a}_{a}.
\end{align}

The exponential generator operator after Jordan-Wigner mapping gives
\begin{widetext}
    \begin{multline}
        U\left( \vec{\theta}\right) = \prod\limits_{abij}\exp \left( \frac{i\theta_{ij}^{ab}}{8}\left[ 
        \begin{array}{c}
        X_{a}X_{b}X_{i}Y_{j}
        +X_{a}X_{b}Y_{i}X_{j}
        +Y_{a}X_{b}Y_{i}Y_{j}
        +X_{a}Y_{b}Y_{i}Y_{j}\\
        -X_{a}Y_{b}X_{i}X_{j}
        -Y_{a}X_{b}X_{i}X_{j}
        -Y_{a}Y_{b}X_{i}Y_{j}
        -Y_{a}Y_{b}Y_{i}X_{j}%
        \end{array}%
        \right] \bigotimes\limits_{v=b}^{a-1}Z_{u}\bigotimes%
        \limits_{u=j}^{i-1}Z_{v}\right),
    \end{multline}
\end{widetext}
which can be easily handled by the Qiskit library.

Now the expectation value of the functional in equation~\eqref{eq:VQE cost function} to be minimised is given by
\begin{equation}
    E_{\text{VQE}}=\min_{\theta }\sum_{a}^{\mathcal{P}}\omega _{a}\left\langle \psi \left( \vec{%
    \theta}\right) \right\vert \hat{P}_{a}\left\vert \psi \left( \vec{\theta}%
    \right) \right\rangle.
\end{equation}

\subsection{optimizers}
The optimizer selected in this study is the simultaneous perturbation stochastic approximation (SPSA)~\cite{Spall1998} for its primary characteristic that makes it well suited for handling noisy measurement.
Optimizer works by iteratively adjusting the parameters of an objective function, with information of the measured objective function, seeking for the optimal set of parameters that optimize the objective function subjected to the given constraints. 
For the case of this study, the objective function is a cost function to be minimized. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Plots_available/plt0025-StateVector_diff_opt.pdf}
    \caption{Training curve using SPSA ran on Statevector simulator.}
    \label{fig:LocalOptimizer_opt_steps}
\end{figure}

A standard stochastic approximation optimizer updates the estimated parameter $\hat{\theta}$ with the form~\cite{Spall1998}
\begin{equation}
    \hat{\theta}_{k+1} = \hat{\theta}_{k} - \hat{a}_k \hat{g}_k\left(\hat{\theta}_{k}\right)
\end{equation}
updating $\hat{\theta}_k$ to $\hat{\theta}_{k+1}$, where $a_k$ is gradient step size factor that tends to $0$ as $k$ tends to a large number.
The simultaneous perturbation stochastic approximation (SPSA) optimizer approximates gradients by performing two cost function evaluations per iteration, perturbing the parameters of the cost function simultaneously in two directions.~\cite{Spall1998}. It has the advantage of handling noisy cost functions, and is capable of handling large dimension cost function.

The implementation of SPSA involve initial setup of the learning rate and perturbation are chosen to be the respective sequences given by
\begin{equation}
    a_{k}=\frac{a}{\left( A+k+1\right) ^{\alpha }},c_{k}=\frac{c}{\left(k+1\right) ^{\gamma }},
\end{equation}
where $k$ is the step number, $a, A, \alpha, c, \gamma$ are positive values.
The value of $\left\{\alpha,\gamma\right\}$ is set to be practical values of $\left\{0.602,0.101\right\}$~\cite{Spall1998}.
\textcolor{red}{ The initial value of perturbation magnitude $c$ is chosen to be 0.1 with prior understanding that solution for $^6$He will not be far from HF solution.}
Finally $A$ is defaulted to be zero and $a$ is calibrated by aiming the first iteration step will move the cost function by 0.1, the calibration is done via the qiskit package.

The fluctuations in minimisation steps arise from the error introduced by near term noisy quantum computer into the process of minimisation.
Termination condition has to be properly considered to define convergence properly.
Our custom termination criteria of our SPSA relies on the logarithm fit of the minimisation steps. 
The minimisation steps are fitted to the equation, 
\begin{equation}
    y = m_k \ln{x} + c_k,
\end{equation}
and the fit is updated on every 10 steps. 
The fitted parameters $m_k$ and $c_k$ are fitted for $x$ from step $1$ to $k$, and $k=\left\{10,20,30,\dots\right\}$
The three criteria that use the fitted $m_k$ are 
\begin{itemize}
    \item Condition 1: $m_k<0$.
    \item Condition 2: $m_{10} < -0.1$
    \item Condition 3: $\frac{\left\|m_{k} - m_{k-10}\right\|}{\left\|m_{k-10}\right\|} \leq 0.1$
\end{itemize}
Condition 1 consider all fitted $m$ are negatives, having the minimizing trend; condition 2 guarantees minimization instead of just random fluctuations in the minimisation; and condition 3 consider small changes in values of $m_{k}$ implies plateauing of the minimization steps.

\section{Results and Discussions\label{sec:Results and discussions}}
Three parts thingy: 
1. Propose a way to terminate minimization to extract meaning full data
2. Table listing 5 repeated computations for each T1T2\&GE combo: obtain average energy (ref log\_240128-01)
3. Table listing the information of all possible combination

\red{Comparing our results with scientific reports paper, our error etc... }. The result focuses on pairing interaction of an Helium-6 nucleus.
This section presents first the pairing interaction computation on a noiseless Statevector simulator, then the computation with noisy quantum computer simulator, and lastly on the discussion of the minimal requirement of a quantum computer to successfully carry out the pairing interaction computation of a $^{6}He$.

\subsection{State-vector Simulations}
Koh:
Starting from different sol, changing initial parameters. 
How different are the converged solution would be if on start from a different intitial parameters 
The choice of initial parameters are {a b c d} because (justification on the intiial parameters)

\subsection{Noisy Simulations}
Simulation of an actual noisy QPU is carried out via the high-performance quantum computing simulation package~\textemdash{qiskit-aer}. From various backends provided, the 16-qubit FakeGuadalupe were chosen for the minimization of the pairing interaction of $^6$He that requires only 12 qubits QPU. Results from other simulated backends with more qubits are presented in the Appendix\ref{Append: otherFakeBackends}.

Discussion on the circuit depth, and how each errors impact on the results.

\subsection{Minimal Requirements for $^6$He Pairing Correlation Simulation\label{sec:fakeJohors}}
Noisy simulators presented too much noise for proper convergence. In this subsection, the minimal requirements of a quantum computer is investigated with a naive approach to improve the quantum computer simulator (colloquially called as "FakeBackend") by increasing the T1 and T2 times, gate error rate, SPAM (state preparation and measurement) error rate, and readout error rate; without in-depth modifications to the other parameters.
We named our simulated noisy quantum computer FakeJohor, and based it on IBM's simulated noisy backend~\textemdash{the 16-qubit FakeGuadalupe}. 

Here the T1 relaxation time (time taken for a qubit to decay from $\left\vert 1\right\rangle$ to $\left\vert 0\right\rangle$), and T2 dephasing time (half life for decoherence of a qubit) are both taken to be the same for all 16 qubit in FakeJohor. The three types of error rates are also taken to be the same at a different values described as follows.

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{plt0031/same_err-hori.png}
%     \includegraphics[width=\textwidth]{plt0031/same_err-vert.png}
%     \caption{FakeJohors with same errors, T1T2 time set different. \red{need to replot this, maybe thicker lines and nicer colours. need  individual explanation for every sub-figures. A: Need to explain what are the colours. B: ... C:.... The first version need to be taller, the height is too short.}}
%     \label{fig:hori-fakejohor-same_err}
% \end{figure*}

\section{Skyrme Effective Interaction}
\label{skyrme two-body interaction}
The effective Skyrme interaction takes the form~\cite{Ryssens2015}
\begin{equation}
\hat{V}\left( \mathbf{r}_{1},\mathbf{r}_{2}\right) =\hat{V}_{C}\left( 
\mathbf{r}_{1},\mathbf{r}_{2}\right) +\hat{V}_{T}\left( \mathbf{r}_{1},%
\mathbf{r}_{2}\right) +\hat{V}_{LS}\left( \mathbf{r}_{1},\mathbf{r}%
_{2}\right) .  \label{Skryme interaction}
\end{equation}%
The density-dependent central two-body Skyrme interaction is defined as%
\begin{eqnarray}
\hat{V}_{C}\left( \mathbf{r}_{1},\mathbf{r}_{2}\right)  &=&t_{0}\left(
1+x_{0}\hat{P}_{\sigma }\right) \delta \left( \mathbf{r}_{1}-\mathbf{r}%
_{2}\right)   \nonumber \\
&&+\frac{1}{2}t_{1}\left( 1+x_{1}\hat{P}_{\sigma }\right) \left[ \mathbf{%
\hat{k}}^{\prime 2}\delta \left( \mathbf{r}_{1}-\mathbf{r}_{2}\right)
+\delta \left( \mathbf{r}_{1}-\mathbf{r}_{2}\right) \mathbf{\hat{k}}^{2}%
\right]   \nonumber \\
&&+t_{2}\left( 1+x_{2}\hat{P}_{\sigma }\right) \mathbf{\hat{k}}^{\prime
}\delta \left( \mathbf{r}_{1}-\mathbf{r}_{2}\right) \mathbf{\hat{k}} 
\nonumber \\
&&+\frac{1}{6}t_{3a}\left( 1+x_{3a}\hat{P}_{\sigma }\right) \rho
_{0}^{\alpha _{a}}\left( \mathbf{R}\right) \delta \left( \mathbf{r}_{1}-%
\mathbf{r}_{2}\right)   \nonumber \\
&&+\frac{1}{6}t_{3b}\left( 1+x_{3b}\hat{P}_{\sigma }\right) \rho
_{0}^{\alpha _{b}}\left( \mathbf{R}\right) \delta \left( \mathbf{r}_{1}-%
\mathbf{r}_{2}\right),   \label{skyrme central dependent}
\end{eqnarray}%
where $\hat{P}_{\sigma }$ is the spin exchange operator, $\mathbf{\hat{k}%
\equiv -}\frac{i}{2}\left( \nabla -\nabla ^{\prime }\right) $ the relative
momentum operator acting to the right and its complex conjugate $\mathbf{%
\hat{k}}^{\prime }$ acting to the left, $\rho _{0}\left( \mathbf{R}\right) $
is the isoscalar density at $\mathbf{R}\equiv \frac{1}{2}\left( \mathbf{r}%
_{1}+\mathbf{r}_{2}\right) $. The spin-orbit part is defined by%
\begin{equation}
\hat{V}_{LS}\left( \mathbf{r}_{1},\mathbf{r}_{2}\right) =iW_{0}\left( 
\mathbf{\hat{\sigma}}_{1}+\mathbf{\hat{\sigma}}_{2}\right) \cdot \mathbf{%
\hat{k}}^{\prime }\times \delta \left( \mathbf{r}_{1}-\mathbf{r}_{2}\right) 
\mathbf{\hat{k}.}  \label{spin orbit part}
\end{equation}%
And the tensor part is defined as%
\begin{eqnarray}
&&\hat{V}_{T}\left( \mathbf{r}_{1},\mathbf{r}_{2}\right)   \nonumber \\
&=&\frac{1}{2}t_{e}\left\{ 
\begin{array}{c}
\left[ 3\left( \mathbf{\sigma }_{1}\cdot \mathbf{k}^{\prime }\right) -\left( 
\mathbf{\sigma }_{1}\cdot \mathbf{\sigma }_{2}\right) \right] \delta \left( 
\mathbf{r}_{1}-\mathbf{r}_{2}\right)  \\ 
+\delta \left( \mathbf{r}_{1}-\mathbf{r}_{2}\right) \left[ 3\left( \mathbf{%
\sigma }_{1}\cdot \mathbf{k}\right) \left( \mathbf{\sigma }_{2}\cdot \mathbf{%
k}\right) -\left( \mathbf{\sigma }_{1}\cdot \mathbf{\sigma }_{2}\right) 
\mathbf{k}^{2}\right] 
\end{array}%
\right\}   \nonumber \\
&&+\frac{1}{2}t_{0}\left\{ 
\begin{array}{c}
\left[ 
\begin{array}{c}
3\left( \mathbf{\sigma }_{1}\cdot \mathbf{k}^{\prime }\right) \delta \left( 
\mathbf{r}_{1}-\mathbf{r}_{2}\right) \left( \mathbf{\sigma }_{2}\cdot 
\mathbf{k}\right)  \\ 
-\left( \mathbf{\sigma }_{1}\cdot \mathbf{\sigma }_{2}\right) \mathbf{k}%
^{\prime }\cdot \delta \left( \mathbf{r}_{1}-\mathbf{r}_{2}\right) \mathbf{k}%
\end{array}%
\right]  \\ 
+\left[ 
\begin{array}{c}
3\left( \mathbf{\sigma }_{2}\cdot \mathbf{k}^{\prime }\right) \delta \left( 
\mathbf{r}_{1}-\mathbf{r}_{2}\right) \left( \mathbf{\sigma }_{1}\cdot 
\mathbf{k}\right)  \\ 
-\left( \mathbf{\sigma }_{1}\cdot \mathbf{\sigma }_{2}\right) \mathbf{k}%
^{\prime }\cdot \delta \left( \mathbf{r}_{1}-\mathbf{r}_{2}\right) \mathbf{k}%
^{\prime }%
\end{array}%
\right] 
\end{array}%
\right\}.   \label{skyrme tensor part}
\end{eqnarray}

The Energy Density Functional of the system is given by 
\begin{equation}
\mathcal{E}_{\text{total}}=\mathcal{E}_{\text{kin}}+\mathcal{E}_{\text{Sk}},
\label{EDF}
\end{equation}%
where the kinetic energy density is given by%
\begin{equation}
\mathcal{E}_{\text{kin}}=\sum\limits_{q=n,p}\frac{\hbar^{2}}{2m_{q}}\tau_{q}\left( \mathbf{r}\right) ,  
\label{kinetic energy density}
\end{equation}%
and the Skyrme energy density is written in the form 
\begin{eqnarray}
\mathcal{E}_{\text{Sk}} &=&\mathcal{E}_{\text{C}}+\mathcal{E}_{\text{T}}+%
\mathcal{E}_{\text{LS}}  \nonumber \\
&=&b_{1}\rho ^{2}+b_{3}\rho \tau +b_{5}\rho \Delta \rho   \nonumber \\
&&+b_{7a}\rho ^{2+\alpha _{a}}+b_{7b}\rho ^{2+\alpha _{b}}+b_{9}\rho \nabla
\cdot \mathbf{J}  \nonumber \\
&&+b_{14}\sum\limits_{\mu ,\nu }J_{\mu \nu }J_{\mu \nu
}+b_{16}\sum\limits_{\mu ,\nu }J_{\mu \nu }J_{\nu \mu }  \nonumber \\
&&+\sum\limits_{q=n,p}\left( 
\begin{array}{c}
b_{2}\rho _{q}^{2}+b_{4}\rho _{q}\tau _{q}+b_{6}\rho _{q}\Delta \rho _{q} \\ 
+b_{8a}\rho ^{\alpha _{a}}\rho _{q}^{2}+b_{8b}\rho ^{\alpha _{b}}\rho
_{q}^{2}+b_{9q}\rho _{q}\nabla \cdot \mathbf{J}_{q} \\ 
+b_{15}\sum\limits_{\mu ,\nu }J_{q,\mu \nu }J_{q,\mu \nu
}+b_{17}\sum\limits_{\mu ,\nu }J_{q,\mu \nu }J_{q,\nu \mu }%
\end{array}%
\right) ,  \label{skyrme energy density}
\end{eqnarray}%
where densities without isospin index are total densities $\rho \left( 
\mathbf{r}\right) \equiv \rho _{p}\left( \mathbf{r}\right) +\rho _{n}\left( 
\mathbf{r}\right) $. The coupling constant are given by%
\begin{eqnarray}
b_{1} &=&\frac{1}{2}t_{0}\left( 1+\frac{x_{0}}{2}\right) ,  \nonumber \\
b_{2} &=&-\frac{1}{2}t_{0}\left( \frac{1}{2}+x_{0}\right) ,  \nonumber \\
b_{3} &=&\frac{1}{4}\left[ t_{1}\left( 1+\frac{x_{1}}{2}\right) +t_{2}\left(
1+\frac{x_{2}}{2}\right) \right] ,  \nonumber \\
b_{4} &=&-\frac{1}{4}\left[ t_{1}\left( \frac{1}{2}+x_{1}\right)
-t_{2}\left( \frac{1}{2}+x_{2}\right) \right] ,  \nonumber \\
b_{5} &=&-\frac{1}{16}\left[ 3t_{1}\left( 1+\frac{x_{1}}{2}\right)
-t_{2}\left( 1+\frac{x_{2}}{2}\right) \right] ,  \nonumber \\
b_{6} &=&\frac{1}{16}\left[ 3t_{1}\left( \frac{1}{2}+x_{1}\right)
+t_{2}\left( \frac{1}{2}+x_{2}\right) \right] ,  \nonumber \\
b_{7a} &=&\frac{1}{12}t_{3a}\left( 1+\frac{x_{3a}}{2}\right) ,  \nonumber \\
b_{8a} &=&-\frac{1}{12}t_{3a}\left( \frac{1}{2}+x_{3a}\right) ,  \nonumber \\
b_{7b} &=&\frac{1}{12}t_{3b}\left( 1+\frac{x_{3b}}{2}\right) ,  \nonumber \\
b_{8b} &=&-\frac{1}{12}t_{3b}\left( \frac{1}{2}+x_{3b}\right) ,  \nonumber \\
b_{9} &=&-\frac{1}{2}W_{0},  \nonumber \\
b_{9q} &=&-\frac{1}{2}W_{0},  \nonumber \\
b_{14} &=&-\frac{1}{8}\left( t_{1}x_{1}+t_{2}x_{2}\right) +\frac{1}{4}\left(
t_{e}+t_{0}\right) ,  \nonumber \\
b_{15} &=&\frac{1}{8}\left( t_{1}-t_{2}\right) -\frac{1}{4}\left(
t_{e}-t_{0}\right) ,  \nonumber \\
b_{16} &=&-\frac{3}{8}\left( t_{e}+t_{0}\right) ,  \nonumber \\
b_{17} &=&\frac{3}{8}\left( t_{e}-t_{0}\right) .
\label{EDF coupling constants}
\end{eqnarray}

